LLM for Comparative Narrative Analysis

In this paper, we conducted a Multi-Perspective Comparative Narrative Analysis (CNA) on three prominent LLMs: GPT-3.5, PaLM2, and Llama2. We applied identical prompts and evaluated their outputs on specific tasks, ensuring an equitable and unbiased comparison between various LLMs. Our study revealed that the three LLMs generated divergent responses to the same prompt, indicating notable discrepancies in their ability to comprehend and analyze the given task. Human evaluation was used as the gold standard, evaluating four perspectives to analyze differences in LLM performance.

==> Sections/3General.tex <==
\section{Dataset}\label{sec:Motivation}

% As we have discussed before, the SOS task is a newly introduced NLP mission, and its benchmark dataset has recently been made available. 
% However, this dataset does not provide the corresponding gold standard for three of the subtasks (except for the overlap task). As a result, we are unable to directly apply any automatic evaluation metrics to assess performance. Consequently, we have opted to rely on human evaluation in this work.

Table \ref{table:allSide} gives an overview of the dataset statistics
created by crawling from AllSides.com \footnote{https://www.allsides.com/} , which consists of news articles covering 2,925 events in total and also has a minimum length of “theme description” to be 15 words. More details can be seen here~\cite{bansal2022semantic}.



\begin{table*}
    \begin{tabular}{|lllll|}
    \hline
    \multicolumn{5}{|c|}{AllSides Dataset: Statistics} \\ \hline
    \multicolumn{1}{|l|}{Split} & \multicolumn{1}{l|}{\#words(per docs)} & \multicolumn{1}{l|}{\#sents(per docs)} & \multicolumn{1}{l|}{\#word (per reference)} & \#sents (per reference) \\ \hline
    \multicolumn{1}{|l|}{Train} & \multicolumn{1}{l|}{1613.69} & \multicolumn{1}{l|}{66.70} & \multicolumn{1}{l|}{67.30} & 2.82 \\ \hline
    
    \multicolumn{1}{|l|}{Test} & \multicolumn{1}{l|}{959.80} & \multicolumn{1}{l|}{44.73} & \multicolumn{1}{l|}{65.46/38.06/21.72/32.82} & 3.65/2.15/1.39/1.52 \\ \hline
    \end{tabular}
    \caption{Statistics for the Training and Testing dataset.}
    \label{table:allSide}
\end{table*}



==> Tables/intersection_examples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reward/Kendall Table

\begin{table*}[!htb]\small
% \begin{subtable}[h]{\textwidth}
\centering


\ra{1.2}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{C{3.5cm} | C{3.5cm} | C{3.5cm} | C{5.5cm}} %| m{0.8cm} | m{2cm}}
\toprule
\multicolumn{4}{c|}{\textbf{Narrative Pair Example \# 1}}\\
\hline
\multicolumn{2}{c|}{\textbf{Narrative 1:} $\mathbf{N_1}$} &
\multicolumn{2}{c}{\textbf{Narrative 2:} $\mathbf{N_2}$} \\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Sample 1
\multicolumn{2}{C{8cm}|}{
% %% -----------------------------------------
%% D1
\hlgreen{
WASHINGTON -- U.S. intelligence and law enforcement agencies have confirmed that President Donald Trump's campaign aides and associates had constant contact with Russian intelligence officials before the election, directly contradicting public statements made by top administration officials. 
}
On Jan. 15, shortly before Trump took office, Vice President Mike Pence repeatedly said on television that there were zero contacts between the campaign and Russian officials. 
$\mathbf{\dotso}$

\hlgreen{
Pence also answered "of course not" when asked a similar question that day by "Fox News Sunday" host Chris Wallace
$\mathbf{\dotso}$

Trump himself also denied these interactions
$\mathbf{\dotso}$

}
"There's nothing that would conclude me that anything different has changed with respect to that time period," Spicer said. 
$\mathbf{\dotso}$

%% -----------------------------------------
} &
\multicolumn{2}{C{8cm}}{
%% -----------------------------------------
%% D2
\hlgreen{
President Trump said Wednesday that new reports saying his associates had contact with Russian officials during last year's campaign are "non-sense"} and accused the U.S. intelligence community of illegally leaking information to news outlets. 
\hlgreen{
"This Russian connection non-sense} is merely an attempt to cover-up the many mistakes made in Hillary Clinton's losing campaign," Mr. Trump tweeted. 
$\mathbf{\dotso}$

Among those supposedly communicating with Russian nationals was former Trump campaign chairman Paul Manafort, the report said. 
\hlgreen{Mr. Manafort denied that he ever knowingly talked to any intelligence official "or anyone}
%% -----------------------------------------
} \\
\hline
\multicolumn{4}{c}{\textbf{Reference Overlap Summaries}} \\\hline
  \multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
  \multicolumn{1}{c}{\textbf{AllSides}}
  \\


\hline
%% A1
President Trump and the Trump administration deny allegations that advisers close to Trump were in constant communication during the campaign with Russians known to US intelligence.
&
%% A2
Trump denied climas that advisers close to him were in "constant communication during the campaign with Russians known to US intelligence.
&
%% A3
Donald Trump and his group claimed that there is no contact with Russian officials during his last year's campaign. 
&
%% A4
Russian intelligence officials made repeated contact with members of President Trump's campaign staff, according to new reports that cite anonymous U.S. officials. American agencies were concerned about the contacts but haven't seen proof of collusion between the campaign and the Russian security apparatus.
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\midrule


\multicolumn{4}{c|}{\textbf{Narrative Pair Example \# 2}}\\\hline
\multicolumn{2}{c|}{\textbf{Narrative 1:} $\mathbf{N_1}$} &
\multicolumn{2}{c}{\textbf{Narrative 2:} $\mathbf{N_2}$} \\
\hline

\multicolumn{2}{C{8cm}|}{
% %% -----------------------------------------
%% D1
John McCain is out of McConnell's clutches for a week or two. 
\hlgreen{
While Sen. John McCain remains in Arizona recovering from Friday's craniotomy, surgery to remove a 5 cm blood clot from above his left eye}, business will not go on as usual in Washington. 
\hlgreen{
Majority Leader Mitch McConnell, who has to have every Republican senator voting to have a prayer of passing Trumpcare, has postponed the vote for the week or two (more likely two) that McCain's recovery will take.
}
That means there's more time for opponents to fight this thing, from the side of all of us trying to keep 22 million people from losing insurance and from the other side. 
$\mathbf{\dotso}$

\hlgreen{With both Paul and Sen. Susan Collins (R-ME) solid "no" votes on the bill}, opponents only need one more out of the eight or so who've expressed reservations about the bill and the secretive, exclusive process McConnell
%% -----------------------------------------
} &
\multicolumn{2}{C{8cm}}{
%% -----------------------------------------
%% D2
\hlgreen{WASHINGTON - The Republican effort to repeal and replace Obamacare faces a major setback as Sen. John McCain, R-Ariz., left the nation's capital for surgery on his eye. 
Over the weekend, Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled Better Care Act vote would be delayed indefinitely because of McCain's absence.}
Subsequently, the Congressional Budget Office (CBO) also delayed its analysis of the bill. 
\hlgreen{With two Republican senators opposed to the measure, McConnell needs as least 50 "yes" votes to pass it.}
\hlgreen{Sen. Rand Paul, R-Ky., says the bill, which keeps taxes on investments and other pieces of Obamacare, doesn't go far enough. 
Moderate Sen. Susan Collins, R-Maine, is also withholding her support because it would slow the rate of growth in spending on Medicaid.}
$\mathbf{\dotso}$

%% -----------------------------------------
} \\
\hline
\multicolumn{4}{c}{\textbf{Reference Overlap Summaries}} \\\hline
\multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
  \multicolumn{1}{c}{\textbf{AllSides}}
  \\


\hline

%% A1
Sen. John McCain remains in Arizona recovering from eye surgery. Senate Majority Leader Mitch  McConnell postponed the vote due to McCain's absence. Two Republican senators opposed to the bill. Possibility of bill failing.
&
%% A2
Sen. John McCain remains unavailable because of the surgery on his eye. Senate Majority Leader Mitch McConnell delayed the vote in his absence. Sen. Rand Paul and Sen. Susan Collins said "no" votes on the bill.
&
%% A3
Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled health care vote would be delayed indefinitely because of McCain's absence.
&
%% A4
Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled Better Care Act vote would be delayed indefinitely because of McCain's absence.
\\
\bottomrule
\end{tabular}
}
\caption{Some examples of \textit{SOS} references from 3 human annotators (\textbf{A\textsubscript{i}}) and the AllSides ``theme-description'' for a given narrative pair $\{N_1, N_2\}$. 
($\mathbf{\dotso}$) denotes some sentences which for not shown for brevity. More examples can be found over \href{https://karmake2.github.io/publications/}{here}. Having multiple human annotators is critical to perform robust evaluation, but it is laborious and time-consuming on humans' part. This also shows that the lack of available datasets is a huge challenge for the SOS task. 
% ($\mathbf{\dotso}$) denotes some the sentences which for not shown for brevity.
}
\label{table:qualitative_analysis}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Tables/prompt_example.tex <==
\begin{table}[]
% \caption{ChatGPT and Bard has different understanding of conflicts in the two narratives}
% \label{table:prompt_example}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cl|}
\hline
\multicolumn{1}{|c|}{Narrative 1} &
  \multicolumn{1}{c|}{Narrative 2} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}.....The indictment against Paul Manafort and his former \\ business associate Rick Gates has been unsealed and \\ leading the list of charges is "Conspiracy Against the\\  United States" and money laundering. "In order to\\  hide Ukraine payments from United States authorities,"\\  the indictment reads.....\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}...Although the indictment with the details has not been unsealed, \\ according to reports Manafort is facing charges on tax fraud and \\ other white collar crimes completely unrelated to the 2016 \\ presidential election. His former business partner, Rick Gates, is \\ also expected to surrender to authorities. Both were told to turn \\ themselves in or face arrest.....\end{tabular} \\ \hline
\multicolumn{2}{|c|}{Prompt: Read the first narrative, then read the second narrative, and highlight the information that two narratives are in conflict with each other} \\ \hline
\multicolumn{1}{|c|}{\textbf{ChatGPT Output}} &
  \multicolumn{1}{c|}{Bard Output} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}After reviewing both narratives, it appears that \\ there is no conflict or contradiction between the two. \\ Instead, the second narrative provides additional information \\ and updates on the situation mentioned in the first narrative, \\ specifically on the charges against Paul Manafort and his \\ surrender to the authorities. Both narratives mention the charges \\ of money laundering and conspiracy against the United States, \\ but the second narrative adds that the charges also include tax fraud \\ and other white-collar crimes unrelated to the 2016 presidential \\ election. Therefore, the second narrative complements and \\ expands on the information presented in the first narrative \\ without contradicting it.\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}The two narratives conflict in the following ways:\\  --The first narrative states that Manafort and Gates were charged with \\      "Conspiracy Against the United States" and money laundering. \\  --The second narrative states that Manafort is facing charges on tax fraud\\      and other white collar crimes completely unrelated to the 2016 presidential election.\\  --The first narrative states that the indictment was unsealed, while the second \\      narrative states that the indictment has not been unsealed.\\  --The first narrative states that Manafort and Gates laundered money through\\    scores of United States and foreign corporations, partnerships, and bank accounts. \\  --The second narrative does not mention any specific allegations of money laundering.\\ It is possible that the two narratives are simply reporting different aspects of\\  the same case. ...\end{tabular} \\ \hline
\end{tabular}%
}
\caption{ChatGPT and Bard has different understanding of conflicts in the two narratives}
\label{table:prompt_example}
\end{table}
